Perfectly to a Tee: Understanding User Perceptions of Personalized LLM-Enhanced Narrative Interventions

Stories about overcoming personal struggles can effectively illustrate the application of psychological theories in real life, yet they may fail to resonate with individuals' experiences. In this work, we employ large language models (LLMs) to create tailored narratives that acknowledge and address unique challenging thoughts and situations faced by individuals. Our study, involving 346 young adults across two settings, demonstrates that personalized LLM-enhanced stories were perceived to be better than human-written ones in conveying key takeaways, promoting reflection, and reducing belief in negative thoughts. These stories were not only seen as more relatable but also similarly authentic to human-written ones, highlighting the potential of LLMs in helping young adults manage their struggles. The findings of this work provide crucial design considerations for future narrative-based digital mental health interventions, such as the need to maintain relatability without veering into implausibility and refining the wording and tone of AI-enhanced content.

==> Section/demography.tex <==
%We recruited 346 participants residing in North America for our study. Of the participants, 172 were students enrolled at a university, recruited through \todo{recruitment}.  Eighty-two students were given the LLM condition, and 90 were given the Non-LLM condition. We assigned each student an ID from 1-172 and refer to them with this ID, prefixed with SL or SN to denote whether they were in the LLM or Non-LLM condition, respectively. There were 142 students who self-identified as male, 25 as female, 2 as other genders, and 3 preferred not to disclose their gender. The students also identified with several racial groups (126 Asian, 19 White, 6 African American, 6 Mixed-Race; 15 preferred not to disclose this information). The students’ ages ranged from 18-27 and their mean age was $20.91 \pm 0.10$.
%The remaining 174 participants were crowdworkers, recruited through \todo{recruitment}. The LLM and Non-LLM conditions had an equal number of crowdworkers, with 87 in the LLM group and 87 in the Non-LLM group. Like with the students, we gave each participant an ID from 1-174, and we refer to them using this ID prefixed with either CL or CN for those in the LLM and Non-LLM conditions, respectively. The crowdworkers identified with several genders (101 female, 63 male, 7 non-binary or third gender, 1 agender; 2 preferred not to disclose). Sixty-eight crowdworkers self-identified as Asian, 65 as White, 13 as African American, 13 as Mixed-Race, and 2 as American Indian or Alaska Native; 13 preferred not to disclose information about their race. The participants in the crowdworkers group were aged 18-29, with a mean age of $22.45 \pm 0.16$.


==> Table/intervention-result.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Your Bolded Caption}}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Column 1} & \textbf{Column 2} & \textbf{Column 3} \\ \hline
Data 1 & Data 2 & Data 3 \\ \hline
Data 4 & Data 5 & Data 6 \\ \hline
Data 7 & Data 8 & Data 9 \\ \hline
\end{tabular}
\end{table}
